Mitigate Parasitic Resistance in Resistive Crossbar-based Convolutional Neural Networks

Traditional computing hardware often encounters on-chip memory bottleneck on large scale Convolution Neural Networks (CNN) applications. With its unique in-memory computing feature, resistive crossbar-based computing attracts researchers' attention as a promising solution to the memory bottleneck issue in von Neumann architectures. However, the parasitic resistances in the crossbar deviate its behavior from the ideal weighted summation operation. In large-scale implementations, the impact of parasitic resistances must be carefully considered and mitigated to ensure circuits' functionality. In this work, we implemented and simulated CNNs on resistive crossbar circuits with consideration of parasitic resistances. Moreover, we carried out a new mapping scheme for high utilization of crossbar arrays on convolution, and a mitigation algorithm to mitigate parasitic resistances in CNN applications. The mitigation algorithm considers parasitic resistances as well as data/kernel patterns of each layer to minimize the computing error in crossbar-based convolutions of CNNs. We demonstrated the proposed methods with implementations of a 4-layer CNN on MNIST and ResNet(20, 32, and 56) on CIFAR-10. Simulation results show the proposed methods well mitigate the parasitic resistances in crossbars. With our methods, modern CNNs on crossbars can preserve ideal(software) level classification accuracy with 6-bit ADCs and DACs implementation.

==> Crossbar_Simulator.tex <==
\subsection{Crossbar Simulator}
So far, simulation tools like MNSIM and NeuroSim+ provide excellent architecture-level analysis.
However, their memristor crossbar models are over simplified. 
%In MNSIM\cite{xia_mnsim:_2016}, an estimated behavior model is used instead of solving node equations; In NeuroSim\cite{chen_neurosim:_2018}, the impact of wire resistance is simplified by adding wire resistance to cross-point devices.
All of these over-simplifications result in unignorable error between predicted output to real output of crossbars. 
And this error become even more severe in large scale implementations. 
In short, coarse modeling of crossbar may be acceptable on power/area/speed estimations, but is questionable on functionality evaluations, such as computing accuracy at layers, or classification accuracy of NN implementations.  
To evaluate NN's functionality on memristor-based implementations, an accurate crossbar simulator is necessary.  
%Recently, two general purpose memristor-based simulation platform have been proposed, MNSIM\cite{xia_mnsim:_2016} and NeuroSim+\cite{chen_neurosim+:_2017}. Both simulation tools can estimate the memristor-based design on the system level, include are, power, and even accuracy. However, both simulation tools adopt over-simplified memristor crossbar model. 

In MNSIM, memrisor-crossbar model been simplified by assume all input voltage($V_{i}$) are the same. Then output voltage $V_{o}$ can be expressed as: $V_{o} = V_{i} \times \frac{R_{s}}{R_{parallel} + R_{s}}$. Here, $R_{parallel}$ represents the resistance of the whole column, $R_{s}$ is the sensing resistance. Assuming, $r$ is the wire resistance between adjacent memristors. Furthermore, the $R_{parallel}$ can be approximatively estimated by $\frac{1}{R_{parallel}} \approx \sum^{M}_{m=1}\frac{1}{R_{m,n} + mr + nr} \approx \frac{M}{R_{min} + (M + N)r}$. M and N is the row/column number of memristor-crossbar respectively. $R_{m,n}$ is the memrisor resistance at intersection of mth row and nth col. $R_{min}$ is the minimum resistance of memristor. For simple input case, MNSIM can give a approximate result which very close to actual result in a very short time. However, due to the over-simplification, such model cannot handle the non-linear property of memristor device. And it may give a very different result, especially when the input voltages are variant. A lot of researchers adopt MNSIM to analysis their memrisor design, but most of their works are focus on area and energy efficiency. A MNSIM-based accuracy analysis on large scale memristor device is still missing.

NeuroSim+ uses bit quantization to represent memristor conductance state. By dividing memristor resistance into finite conductance state, NeuroSim+ reduced the complexity of crossbar model at the cost of accuracy loss. Similar with MNSIM, NeuroSim+ still not consider non-linear issue and realistic circuit interaction effect. NeuroSim+ based memristor design verification also focus on area, and power efficiency. 

Recently, Yi Cai et.al\cite{cai_training_2018} proposed using memristor-crossbar architecture to perform matrix operation in CNN and tested their proposed framework on ResNet-20 with CIFAR10 dataset. However, they still use bit quantization to represent memristor resistance. And the non-linear property is considered as a Gaussian noise when update the memristor resistance. Such assumption make the model still in a very high level hierarchy, doesn't deal with the detailed circuit issue. Moreover, such work only discussed how to use memristor device for online-learning. How to leverage memristor device for off-line learning(include transferring and mapping pre-trained NN weights) on large scale network and dataset is still vague. 

To show the practicability of a memristor-based design, accuracy verification is much more important than area, and power efficiency. Both above simulation platforms adopt simplified crossbar circuit model which limits their scalability on accuracy aspect. Although SPICE can be used to do full circuit simulation by adopting memristor model, it is not practical on large scale memristor array and input dataset due to its low speed. 
%Dot-Product Engine\cite{hu_dot-product_2016} is a promising tool can be used to address above issues. 

An ideal crossbar simulator should give reasonable accurate result in affordable time effort.
Here We adapt the experiment-verified memristor crossbar simulator from \cite{hu_memristor-based_2018}.
The simulator uses realistic device models, solve node equations with consideration of wire resistance and other circuit parameters, then finally verified with experiment result at large scales.
Fig.\ref{fig_1T1Msim} illustrates the simulation result of the memristor crossbar simulator, which is verified with experiment up to $128 \times 64$.

Besides the simulator, the conversion algorithm, as a mapping method is employed to improve VMM computing accuracy with consideration of wire resistance and device nonlinearity\cite{hu_dot-product_2016}.
%Comparing to linear mapping, it uses a specific conversion signal $V_{conv}$ as input, and calculates the crossbar conductance so that the ideal current per cross-point for $V_{conv}$ can be achieved in the realistic crossbar array. 
The conversion algorithm uses a conversion signal $V_{conv}$ to find a new conductance mapping $G'$, so that
$$
VG \approx \mathrm{CrossbarSim}(V, G')
$$
where CrossbarSim() is the realistic crossbar model. 
%With the conversion algorithm,  a realistic crossbar with $G'$ can perform as an ideal crossbar with $G$ for input $V_{conv}$, and with approximated output for other input $V$. 
Although the original conversion algorithm provides 7$\sim$8 bit-accuracy result for general VMM, it does not consider impact of data/weight patterns in specific applications, which may affect its performance significantly. 
%With DPE and its conversion algorithm, memristor crossbar can be treat as a general vector-matrix multiplier. By solving node equation with considering wire resistance and other circuit parameters for every intersection, it can give us a actual experimental verified result. Associated conversion algorithm can fine-tuning memristor conductance to make the actual result more close to ideal mathematic result. 

%Although DPE has so many merits, it still has disadvantage. Firstly, as a general purpose VMM it doesn't consider the impact of input or matrix pattern. Secondly, for multi-level cascaded memristor crossbar, the error accumulation/penetration has not been studied yet. 


==> JETC (Final version)/Crossbar_Simulator.tex <==
\subsection{Crossbar Simulator}
So far, simulation tools like MNSIM and NeuroSim+ provide excellent architecture-level analysis.
However, their memristor crossbar models are over simplified. 
%In MNSIM\cite{xia_mnsim:_2016}, an estimated behavior model is used instead of solving node equations; In NeuroSim\cite{chen_neurosim:_2018}, the impact of wire resistance is simplified by adding wire resistance to cross-point devices.
All of these over-simplifications result in unignorable error between predicted output to real output of crossbars. 
And this error become even more severe in large scale implementations. 
In short, coarse modeling of crossbar may be acceptable on power/area/speed estimations, but is questionable on functionality evaluations, such as computing accuracy at layers, or classification accuracy of NN implementations.  
To evaluate NN's functionality on memristor-based implementations, an accurate crossbar simulator is necessary.  
%Recently, two general purpose memristor-based simulation platform have been proposed, MNSIM\cite{xia_mnsim:_2016} and NeuroSim+\cite{chen_neurosim+:_2017}. Both simulation tools can estimate the memristor-based design on the system level, include are, power, and even accuracy. However, both simulation tools adopt over-simplified memristor crossbar model. 

In MNSIM, memrisor-crossbar model been simplified by assume all input voltage($V_{i}$) are the same. Then output voltage $V_{o}$ can be expressed as: $V_{o} = V_{i} \times \frac{R_{s}}{R_{parallel} + R_{s}}$. Here, $R_{parallel}$ represents the resistance of the whole column, $R_{s}$ is the sensing resistance. Assuming, $r$ is the wire resistance between adjacent memristors. Furthermore, the $R_{parallel}$ can be approximatively estimated by $\frac{1}{R_{parallel}} \approx \sum^{M}_{m=1}\frac{1}{R_{m,n} + mr + nr} \approx \frac{M}{R_{min} + (M + N)r}$. M and N is the row/column number of memristor-crossbar respectively. $R_{m,n}$ is the memrisor resistance at intersection of mth row and nth col. $R_{min}$ is the minimum resistance of memristor. For simple input case, MNSIM can give a approximate result which very close to actual result in a very short time. However, due to the over-simplification, such model cannot handle the non-linear property of memristor device. And it may give a very different result, especially when the input voltages are variant. A lot of researchers adopt MNSIM to analysis their memrisor design, but most of their works are focus on area and energy efficiency. A MNSIM-based accuracy analysis on large scale memristor device is still missing.

NeuroSim+ uses bit quantization to represent memristor conductance state. By dividing memristor resistance into finite conductance state, NeuroSim+ reduced the complexity of crossbar model at the cost of accuracy loss. Similar with MNSIM, NeuroSim+ still not consider non-linear issue and realistic circuit interaction effect. NeuroSim+ based memristor design verification also focus on area, and power efficiency. 

Recently, Yi Cai et.al\cite{cai_training_2018} proposed using memristor-crossbar architecture to perform matrix operation in CNN and tested their proposed framework on ResNet-20 with CIFAR10 dataset. However, they still use bit quantization to represent memristor resistance. And the non-linear property is considered as a Gaussian noise when update the memristor resistance. Such assumption make the model still in a very high level hierarchy, doesn't deal with the detailed circuit issue. Moreover, such work only discussed how to use memristor device for online-learning. How to leverage memristor device for off-line learning(include transferring and mapping pre-trained NN weights) on large scale network and dataset is still vague. 

To show the practicability of a memristor-based design, accuracy verification is much more important than area, and power efficiency. Both above simulation platforms adopt simplified crossbar circuit model which limits their scalability on accuracy aspect. Although SPICE can be used to do full circuit simulation by adopting memristor model, it is not practical on large scale memristor array and input dataset due to its low speed. 
%Dot-Product Engine\cite{hu_dot-product_2016} is a promising tool can be used to address above issues. 

An ideal crossbar simulator should give reasonable accurate result in affordable time effort.
Here We adapt the experiment-verified memristor crossbar simulator from \cite{hu_memristor-based_2018}.
The simulator uses realistic device models, solve node equations with consideration of wire resistance and other circuit parameters, then finally verified with experiment result at large scales.
Fig.\ref{fig_1T1Msim} illustrates the simulation result of the memristor crossbar simulator, which is verified with experiment up to $128 \times 64$.

Besides the simulator, the conversion algorithm, as a mapping method is employed to improve VMM computing accuracy with consideration of wire resistance and device nonlinearity\cite{hu_dot-product_2016}.
%Comparing to linear mapping, it uses a specific conversion signal $V_{conv}$ as input, and calculates the crossbar conductance so that the ideal current per cross-point for $V_{conv}$ can be achieved in the realistic crossbar array. 
The conversion algorithm uses a conversion signal $V_{conv}$ to find a new conductance mapping $G'$, so that
$$
VG \approx \mathrm{CrossbarSim}(V, G')
$$
where CrossbarSim() is the realistic crossbar model. 
%With the conversion algorithm,  a realistic crossbar with $G'$ can perform as an ideal crossbar with $G$ for input $V_{conv}$, and with approximated output for other input $V$. 
Although the original conversion algorithm provides 7$\sim$8 bit-accuracy result for general VMM, it does not consider impact of data/weight patterns in specific applications, which may affect its performance significantly. 
%With DPE and its conversion algorithm, memristor crossbar can be treat as a general vector-matrix multiplier. By solving node equation with considering wire resistance and other circuit parameters for every intersection, it can give us a actual experimental verified result. Associated conversion algorithm can fine-tuning memristor conductance to make the actual result more close to ideal mathematic result. 

%Although DPE has so many merits, it still has disadvantage. Firstly, as a general purpose VMM it doesn't consider the impact of input or matrix pattern. Secondly, for multi-level cascaded memristor crossbar, the error accumulation/penetration has not been studied yet. 

